A parallel sweeping preconditioner for heterogeneous 3D Helmholtz equations

A parallelization of a sweeping preconditioner for 3D Helmholtz equations without large cavities is introduced and benchmarked for several challenging velocity models. The setup and application costs of the sequential preconditioner are shown to be O({\gamma}^2 N^{4/3}) and O({\gamma} N log N), where {\gamma}({\omega}) denotes the modestly frequency-dependent number of grid points per Perfectly Matched Layer. Several computational and memory improvements are introduced relative to using black-box sparse-direct solvers for the auxiliary problems, and competitive runtimes and iteration counts are reported for high-frequency problems distributed over thousands of cores. Two open-source packages are released along with this paper: "Parallel Sweeping Preconditioner (PSP)" and the underlying distributed multifrontal solver, "Clique".

==> Makefile <==
DOC=sisc12-sweeping

$(DOC).pdf: $(DOC).tex tikz/plane-with-single-pml.tex \
                       tikz/auxiliary.tex \
                       tikz/boundary.tex \
                       tikz/sep-tree.tex \
                       tikz/subteam.tex \
                       pdf/overthrust.pdf \
                       mc_mr.tex \
                       partial_matrix.tex \
                       vector.tex \
                       overthrust-test.tex
	pdflatex $<
	pdflatex $<

clean:
	rm -f $(DOC).pdf *.aux *.log *.toc *.vrb *.snm *.out 


==> convergence-old.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{r|c|c|c|c|c|}
\cline{2-6}
 & \multicolumn{5}{|c|}{velocity model} \\
\cline{2-6}
  & barrier & wedge & two-layers & waveguide & Overthrust  \\
\hline
\multicolumn{1}{|r|}{Hz}
  & 50 & 75 & 50 & 37.5 & 8 \\
\hline
\multicolumn{1}{|r|}{PML amplitude}
  & 3.0 & 4.0 & 4.0 & 2.0 & 7.5 \\
\hline
\multicolumn{1}{|r|}{damping}
  & 7.0 & 7.0 & 7.0 & 7.0 & 7.07 \\
\hline
\multicolumn{1}{|r|}{\# of its.}
  & 28 & 49 & 48 & 52 & 72  \\
\hline
\end{tabular}
\caption{The number of iterations required for convergence for five model 
problems. For the first four velocity models, the grid size was $500^3$ and 
roughly 50 wavelengths were spanned in each direction, whereas the Overthrust
grid was $801 \times 801 \times 187$ and spanned roughly 73 wavelengths in the 
$x_1$ and $x_2$ directions and 17 wavelengths in the vertical direction. In all 
cases, five grid points were used for all PML discretizations and four planes
were processed per panel.}
\label{tbl:convergence}
\end{table}



==> partial_matrix_old.tex <==
\begin{figure}
\centering
$
\left(\begin{array}{ccc}
 \{0,2,4\} & \{0,2,4\} & \{0,2,4\} \\
 \{1,3,5\} & \{1,3,5\} & \{1,3,5\} \\
 \{0,2,4\} & \{0,2,4\} & \{0,2,4\} \\
 \{1,3,5\} & \{1,3,5\} & \{1,3,5\} \\
 \{0,2,4\} & \{0,2,4\} & \{0,2,4\} \\
 \{1,3,5\} & \{1,3,5\} & \{1,3,5\} \\
 \{0,2,4\} & \{0,2,4\} & \{0,2,4\} 
\end{array}\right),\;\;\;\;\;\;
\left(\begin{array}{ccc}
 \{0,1\} & \{0,1\} & \{0,1\} \\
 \{2,3\} & \{2,3\} & \{2,3\} \\
 \{4,5\} & \{4,5\} & \{4,5\} \\
 \{0,1\} & \{0,1\} & \{0,1\} \\
 \{2,3\} & \{2,3\} & \{2,3\} \\
 \{4,5\} & \{4,5\} & \{4,5\} \\
 \{0,1\} & \{0,1\} & \{0,1\} 
\end{array}\right)
$
\caption{Overlay of the owning process ranks of a 7 $\times$ 3 matrix 
distributed over a 2 $\times$ 3 process grid in the $[M_C,\star]$ 
distribution (left) and the $[M_R,\star]$ distribution (right).}
\label{fig:partial_matrix}
\end{figure}


==> vector_old.tex <==
\begin{figure}
\centering
$
\left(\begin{array}{ccc}
 0 & 0 & 0 \\
 1 & 1 & 1 \\
 2 & 2 & 2 \\
 3 & 3 & 3 \\
 4 & 4 & 4 \\
 5 & 5 & 5 \\
 0 & 0 & 0 
\end{array}\right),\;\;\;\;\;\;
\left(\begin{array}{ccc}
 0 & 0 & 0 \\
 2 & 2 & 2 \\
 4 & 4 & 4 \\
 1 & 1 & 1 \\
 3 & 3 & 3 \\
 5 & 5 & 5 \\
 0 & 0 & 0 
\end{array}\right)
$
\caption{Overlay of the owning process ranks of a 7 $\times$ 3 matrix 
distributed over a 2 $\times$ 3 process grid in the $[V_C,\star]$ vector 
distribution (left) and the $[V_R,\star]$ vector distribution (right).}
\label{fig:vector}
\end{figure}


==> weak-scaling-mid.tex <==
\begin{table}
\footnotesize
\centering
% Only 32, 256, and 3072 proc cases have new affinity results!!!
\begin{tabular}{r|c|c|c|c|c|c|c|}
\cline{2-8}
 & \multicolumn{7}{|c|}{number of processes} \\
\cline{2-8}
                       & 32 & 64 & 128 & 256 & 512 & 1024 & 2048  \\
\hline
\multicolumn{1}{|r|}{grid}
                       & $201 \!\times\! 201 \!\times\! 47$
                       & $254 \!\times\! 254 \!\times\! 60$
                       & $320 \!\times\! 320 \!\times\! 75$
                       & $401 \!\times\! 401 \!\times\! 94$
                       & $506 \!\times\! 506 \!\times\! 119$
                       & $637 \!\times\! 637 \!\times\! 150$
                       & $801 \!\times\! 801 \!\times\! 187$ \\
\hline
\multicolumn{1}{|r|}{setup}
                       & 26.07 (25.52) 
                       & 35.50 (34.91)
                       & 48.40 (46.23)
                       & 66.33 (63.41) 
                       & 92.95 (86.90)
                       & 130.4 (120.6)
                       & 193.0 (175.2) \\
\hline
\multicolumn{1}{|r|}{apply}
                       & 1.40 (1.66) 
                       & 1.70 (2.70)
                       & 1.87 (4.26)
                       & 2.20 (5.11) 
                       & 2.58 (9.61)
                       & 2.80 (13.3)
                       & 3.52 (24.5) \\
\hline
\end{tabular}
\caption{Timings (in seconds) on TACC's Lonestar for the SEG/EAGE Overthrust 
model, where timings in parentheses do not make use of selective inversion.
All cases used a complex double-precision second-order finite-difference 
stencil with 5 grid spacings of PML for all boundaries and the auxiliary 
problems. 
The preconditioner was configured with four planes per panel and 8 processes 
per node.
The `apply' timings refer to a single application of the preconditioner to 
four right-hand sides.}
\label{tbl:weak-scaling}
\end{table}



==> weak-scaling-old.tex <==
\begin{table}
\centering
% Only 32, 256, and 3072 proc cases have new affinity results!!!
\begin{tabular}{r|c|c|c|}
\cline{2-4}
 & \multicolumn{3}{|c|}{number of processes} \\
\cline{2-4}
                       & 32    & 256   & 2048  \\
\hline
\multicolumn{1}{|r|}{Hz}
                       & 2  & 4 & 8 \\
\hline
\multicolumn{1}{|r|}{grid size}
                       & $201 \!\times\! 201 \!\times\! 47$
                       & $401 \!\times\! 401 \!\times\! 94$
                       & $801 \!\times\! 801 \!\times\! 187$ \\
\hline
\multicolumn{1}{|r|}{setup [sec]}
                       & 26.07 (25.52) & 66.33 (63.41) & 193.0 (175.2) \\
\hline
\multicolumn{1}{|r|}{apply [sec]}
                       & 1.40 (1.66) & 2.20 (5.11) & 3.52 (24.5) \\
\hline
\end{tabular}
\caption{Weak scaling results on TACC's Lonestar for the SEG/EAGE Overthrust 
model, where timings in parentheses do not make use of selective inversion.
All cases used a complex double-precision second-order finite-difference 
stencil with 5 grid spacings of PML for all boundaries and the auxiliary 
problems. 
The preconditioner was configured with four planes per panel and 8 processes 
per node.
The `apply' timings refer to a single application of the preconditioner to 
four right-hand sides.}
\label{tbl:weak-scaling}
\end{table}


